"Laughing at you or with you": The Role of Sarcasm in Shaping the Disagreement Space

Detecting arguments in online interactions is useful to understand how conflicts arise and get resolved. Users often use figurative language, such as sarcasm, either as persuasive devices or to attack the opponent by an ad hominem argument. To further our understanding of the role of sarcasm in shaping the disagreement space, we present a thorough experimental setup using a corpus annotated with both argumentative moves (agree/disagree) and sarcasm. We exploit joint modeling in terms of (a) applying discrete features that are useful in detecting sarcasm to the task of argumentative relation classification (agree/disagree/none), and (b) multitask learning for argumentative relation classification and sarcasm detection using deep learning architectures (e.g., dual Long Short-Term Memory (LSTM) with hierarchical attention and Transformer-based architectures). We demonstrate that modeling sarcasm improves the argumentative relation classification task (agree/disagree/none) in all setups.

==> attn.tex <==
Figures \ref{figure:lstmcomp1} and \ref{figure:lstmcomp2} show the heat maps of the attention weights of $LSTM_{attn}$ \emph(left) and $LSTM_{mt}$ \emph{right} models for two particular turn pairs, respectively. In Figure \ref{figure:lstmcomp1} we observe that the $LSTM_{attn}$ gives identical weights to the words in $pt$ whereas words that seem to make argumentative claims (e.g., ``you actually think'') receive high weights in $ct$. In contrary, in  $LSTM_{MT}$ words such as ``primate'' ($pt$) $\leftrightarrow$ ``evolution'', ``creatures''receive highest weights showing it is learning the correlation of these terms. We also observe sarcasm markers such as ``ya'', ``oops'' and multiple exclamation receive high attention weight showing how the multi-task model is able to bring sarcasm information for correctly classifying the turn pair. 



